On the Role of Feedback in Test-Time Scaling of Agentic AI Workflows

Agentic AI workflows (systems that autonomously plan and act) are becoming widespread, yet their task success rate on complex tasks remains low. A promising solution is inference-time alignment, which uses extra compute at test time to improve performance. Inference-time alignment relies on three components: sampling, evaluation, and feedback. While most prior work studies sampling and automatic evaluation, feedback remains underexplored. To study the role of feedback, we introduce Iterative Agent Decoding (IAD), a procedure that repeatedly inserts feedback extracted from different forms of critiques (reward models or AI-generated textual feedback) between decoding steps. Through IAD, we analyze feedback along four dimensions: (1) its role in the accuracy-compute trade-offs with limited inference budget, (2) quantifying the gains over diversity-only baselines such as best-of-N sampling, (3) effectiveness of composing feedback from reward models versus textual critique, and (4) robustness to noisy or low-quality feedback. Across Sketch2Code, Text2SQL, Intercode, and WebShop, we show that IAD with proper integration of high fidelity feedback leads to consistent gains up to 10 percent absolute performance improvement over various baselines such as best-of-N. Our findings underscore feedback as a crucial knob for inference-time alignment of agentic AI workflows with limited inference budget.

==> intro_old.tex <==
AI agents demonstrate remarkable potential across a wide range of applications, but still face challenges in tasks that require multimodal understanding, strategic planning, and reasoning. For example, in complex agentic tasks such as \textbf{Sketch2Code} \citep{li2024sketch2codeevaluatingvisionlanguagemodels}, \textbf{Text2SQL} \citep{li2024can}, \textbf{Intercode} \citep{intercode} and \textbf{Webshop} \citep{yao2023webshopscalablerealworldweb},  state-of-the-art AI agents can only achieve 20–30\% accuracy. Post-training via SFT and RL \citep{rlhf1, rlhf2, rlhf3} has been an effective tool to enhance the capabilities of generative models; however, it is not directly applicable to AI agents due to their inherently black box nature because of their operation in environments with no access to the internals~\citep{agent2, agent1}.  Hence, we focus on inference-time approaches which are (i) API-friendly (applicable to closed-source models accessible via commercial APIs) and (ii) compatible with various underlying models.



\noindent \textbf{Inference-time AI agent alignment:}  Broadly, test-time scaling consists of iteration over three key components: \textit{sampling}, \textit{evaluation}, and \textit{feedback} as illustrated in Figure \ref{fig:inf_bb}. A typical inference-time iteration involves sampling one or more outcomes from the generative model, evaluating them using a judge/reward, and then generating feedback to improve subsequent outcomes. The role of \textit{sampling} and \textit{evaluation} is well-studied in literature with efficient and scalable algorithms based on best-of-N (BoN) approaches \citep{nakano2021webgpt,bon3}. BoN-based approaches operate by sampling multiple responses and selecting the best according to a verifier, effectively leveraging the sampling and evaluation steps. However, a key limitation of BoN approaches is their inability to incorporate feedback mechanisms for iterative refinement. 



\noindent While BoN and variants \citep{nakano2021webgpt, bon3, verdun2025soft} are highly parallelizable allowing responses to be sampled and evaluated concurrently to reduce wall-clock latency—it may not be compute-optimal. That is, to achieve a desirable outcome, BoN may require generating a large number of samples and evaluating each independently. This parallelism trades off compute efficiency for lower latency. In contrast, we focus on inference-time alignment strategies designed to maximize performance under a fixed compute budget, where compute is defined concretely as the total number of API calls or forward passes through the model. In such compute-constrained settings, incorporating feedback becomes critical for effective test-time scaling. Thus, while BoN strikes a balance between latency and compute, approaches that leverage feedback are better suited when compute is the principal focus.



\begin{figure*}[t]

    \centering

    \includegraphics[width=0.9\textwidth]{figs/flow_algo4.png}

     \caption{Overview of Iterative Agent Decoding (IAD), highlighting the sampling, evaluation, and feedback components of inference-time alignment. The figure illustrates how feedback is constructed from verification signals and used to iteratively refine model outputs.} 

    \label{fig:overall}

\end{figure*}



\noindent \textbf{Beyond Sampling in Inference Alignment} :  Recently, several sequential approaches have emerged \citep{refine1, tryagain, selfdebug, robeyns2025selfimprovingcodingagent, jiang2024selfplanningcodegenerationlarge} that aim to integrate feedback mechanisms primarily using self-LLMs as judges such as self-refine \citep{refine1} where models iteratively improve their outputs based on self-critique, and try-again strategies \citep{tryagain} that prompt the LLM to generate alternative responses when initial attempts fail. Other approaches include \citep{selfdebug}, where LLMs identify and correct errors in their own generated code. Additionally, recent advancements in agentic systems have show-cased their ability to self-improve \citep{robeyns2025selfimprovingcodingagent, jiang2024selfplanningcodegenerationlarge} These approaches, along with other heuristically driven refinement and verification techniques, highlight a growing trend towards more adaptive approaches. 



\noindent However, existing works often lack a focused analysis of how feedback should be designed, integrated, or optimized. While prior approaches \citep{selfdebug, tryagain, refine1} demonstrate the utility of adaptive learning with feedback, a clear understanding of the mechanisms by which LLMs learn from this feedback, especially with scalar feedback or score, is still developing. As a result, the role of feedback in inference-time alignment, especially in black-box agentic environments, remains under-examined. We aim to address this gap by focusing on feedback and systematically understanding its impact on test-time scaling of agentic workflows.





\noindent \textbf{Understanding the role of feedback:} To understand the role and impact of feedback on inference-time alignment, we require a unified framework that flexibly integrates diverse forms of feedback, guided by a verifier, without relying heavily on prompt engineering, which can be costly and fragile. To this end, we introduce Iterative Agent Decoding (IAD), a sequential framework designed to incorporate various forms of feedback to understand the role of feedback in inference-time alignment of agents. Through IAD we uncover several intriguing results, detailed below.



\noindent \textbf{1. Accuracy vs compute: budget-constrained scaling with feedback:} We demonstrate that feedback plays a critical role in budget-constrained settings and helps achieve up to a 10\% accuracy gain over strong feedback-free baselines with the same budget. However, this margin narrows with increased budget, which allows for generation of more candidates (e.g., larger $N$ is BoN) or using more capable models like increased model complexity from Gemini-1.5 to Gemini-2.0 and Gemini-2.5 as shown in Figure \ref{fig:mainfig_sk2code}.



\noindent \textbf{2. Impact of adaptive feedback beyond sampling gain:} We perform controlled experiments to capture the gains from feedback beyond the diversity gains from sampling. Our results demonstrate that the gains in IAD arise from adaptive, feedback-guided refinement yielding performance improvements of 4–8\% in both Sketch2Code and Text2SQL. This also highlights that feedback plays a crucial role in agentic tasks and scenarios where sampling diversity is low.



\noindent \textbf{3. Design and role of feedback form:} We investigate the impact of different forms of feedback - primarily scalar and textual on inference-time alignment. Textual feedback is relatively straightforward to integrate, as it can be directly incorporated into the model prompt. However, designing effective feedback from scalar rewards and preferences remains underexplored. In IAD, we focus on methods to extract useful signal from scalar rewards and demonstrate that the performance gains crucially depend on the design of proper feedback. Our experiments show that transforming scalar feedback into directional prompts yields performance gains of up to 6–7\% over baselines in Sketch2Code and Text2SQL.



\noindent \textbf{4. Sensitivity to feedback quality:} We study the sensitivity and robustness of inference alignment to feedback quality via controlled sparsity and noise in feedback signals. We see that IAD remains effective under moderate degradation, but its performance declines with increasing noise. Under high sparsity or heavy noise, the performance gains over sampling-based methods drop by approximately 4–5\%, highlighting the importance of feedback fidelity for reliable test-time scaling.
